A Closed-Form Uncertainty Propagation in Non-Rigid Structure from Motion

Semi-Definite Programming (SDP) with low-rank prior has been widely applied in Non-Rigid Structure from Motion (NRSfM). Based on a low-rank constraint, it avoids the inherent ambiguity of basis number selection in conventional base-shape or base-trajectory methods. Despite the efficiency in deformable shape reconstruction, it remains unclear how to assess the uncertainty of the recovered shape from the SDP process. In this paper, we present a statistical inference on the element-wise uncertainty quantification of the estimated deforming 3D shape points in the case of the exact low-rank SDP problem. A closed-form uncertainty quantification method is proposed and tested. Moreover, we extend the exact low-rank uncertainty quantification to the approximate low-rank scenario with a numerical optimal rank selection method, which enables solving practical application in SDP based NRSfM scenario. The proposed method provides an independent module to the SDP method and only requires the statistic information of the input 2D tracked points. Extensive experiments prove that the output 3D points have identical normal distribution to the 2D trackings, the proposed method and quantify the uncertainty accurately, and supports that it has desirable effects on routinely SDP low-rank based NRSfM solver.

==> defines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal packages
% \usepackage{bmpsize}
\usepackage{amsthm}
\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage{amsmath,amssymb,enumerate}
\usepackage{mathrsfs}
\usepackage{times}
\usepackage{multicol}
\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{balance}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dblfloatfix} 
\usepackage{bbold}
\usepackage{makecell}
\usepackage{hhline} % double-line in a table
\usepackage{float} % Places the float at precisely the location in the code
\usepackage[mathscr]{euscript}
\usepackage[noadjust]{cite} % to group references
\usepackage[numbers]{natbib}

\usepackage{comment}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{soul} 
% \usepackage{ulem} % Strikethrough in Section Title 
\usepackage{balance}
\usepackage{dsfont} % indicator function
% \usepackage{physics} % partial differential equation
\usepackage{setspace} % double spacing
\usepackage{accents} % widetilde
% \usepackage[style=numeric-comp]{biblatex}

% \usepackage{graphicx}
% \usepackage{fixltx2e}


% packages with options
%\usepackage[dvipdfmx]{graphicx} 
\usepackage[T1]{fontenc}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage[utf8]{inputenc}
% \usepackage[title]{appendix}


% packages with setups
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
}

\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
% \let\proof\relax 
% \let\endproof\relax

% \addtolength{\skip\footins}{0.5pc plus 5pt minus 2pt} % white space above footnotes

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Graphics path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{
    {fig/}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}

% proof style
\renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm inputs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{red}{Maani: #1}}}]}
% \definecolor{note}{rgb}{0.3,0.7,0.25}
% \definecolor{rephase}{rgb}{0.8,0.3,0.3}
% \definecolor{bag}{rgb}{0.6,0.6,0.2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functionalities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squeezeup}{\vspace{-3mm}} % save space



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematics Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \def\realnumbers{\mathbb{R}}
% \def\real{\mathbb{R}}
% \def\reals{\mathbb{R}}

\newcommand{\transpose}{\mathsf{T}}


% Groups and Algebra
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\Sim}{\mathrm{Sim}}
\newcommand{\Exp}{\mathrm{Exp}}
\newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}

% \DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
% \DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
% \DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}


% \newcommand{\GL}{\mathrm{GL}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\m}{\mathop{\mathrm{m}}}
\newcommand{\rad}{\mathop{\mathrm{rad}}}
\newcommand{\dBm}{\mathop{\mathrm{dBm}}}
\newcommand{\Hz}{\mathop{\mathrm{Hz}}}
\newcommand{\GHz}{\mathop{\mathrm{GHz}}}
\newcommand{\MHz}{\mathop{\mathrm{MHz}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
% \newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
% \newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


% lowers
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands for letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
% \DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
% \DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% % \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
% \DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
% \DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
% \DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
% \DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
% % \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
% \DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% % \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
% \DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
% \DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
% \DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
% \DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
% \DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
% % \DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}


% % lowers
% \DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
% \DeclareDocumentCommand{\n}{ O{} O{} }{\textbf{n}_{#1}^{#2}}
% \DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
% \DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
% \DeclareDocumentCommand{\q}{ O{} O{} }{\textbf{q}_{#1}^{#2}}
% \DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
% \DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
% \DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}


\makeatletter
\newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
\newcommand{\mathcenter}{\@fleqnfalse}
\makeatother

